ETHIC: Evaluating Large Language Models on Long-Context Tasks with High Information Coverage

Recent advancements in large language models (LLM) capable of processing extremely long texts highlight the need for a dedicated evaluation benchmark to assess their long-context capabilities. However, existing methods, like the needle-in-a-haystack test, do not effectively assess whether these models fully utilize contextual information, raising concerns about the reliability of current evaluation techniques. To thoroughly examine the effectiveness of existing benchmarks, we introduce a new metric called information coverage (IC), which quantifies the proportion of the input context necessary for answering queries. Our findings indicate that current benchmarks exhibit low IC; although the input context may be extensive, the actual usable context is often limited. To address this, we present ETHIC, a novel benchmark designed to assess LLMs' ability to leverage the entire context. Our benchmark comprises 1,986 test instances spanning four long-context tasks with high IC scores in the domains of books, debates, medicine, and law. Our evaluations reveal significant performance drops in contemporary LLMs, highlighting a critical challenge in managing long contexts. Our benchmark is available at https://github.com/dmis-lab/ETHIC.

==> tables/prompt_template.tex <==
\begin{table*}[t]
\centering
\footnotesize
\begin{tabular}{p{15cm}}
\toprule
Your task is to refine responses to patient inquiries gathered from an online medical consultation platform to mirror the natural communication style of a practicing healthcare expert. You also should remove noise from responses, including patients' or doctors' names, unintended text generated during data crawling, and mentions of specific platforms (e.g., Chat Doctor). 
Refer to the following examples.
\\\\
Original text: Dear Friend. Welcome to Chat Doctor. I am Chat Doctor. I understand your concern. Recurring yeast / final infection occur due to:1. Improper treatment.2. Inadequate treatment3. Wrong diagnosis.4. Not treating the partner. I would advise you to get a Urine examination done for bacteria and fungus. When the reports are available, get treated. Also, treat your partner. This is my personal opinion for you based on available details. If you have any further query please ask me. Stay HealthyChatDoctor, MD
\\\\
Modified text: I understand your concern regarding recurrent yeast/fungal infections. Several factors can contribute to this issue, including improper or inadequate treatment, misdiagnosis, or failure to treat the partner. I recommend getting a urine examination done to check for bacteria and fungus. Once the reports are available, appropriate treatment can be initiated. It's also important to ensure that your partner receives treatment if necessary. Please note that this advice is based on the information provided. If you have any further questions or concerns, feel free to ask. Take care and stay healthy.
\\\\
Original text: Hi, dairy have gone through your question. I can understand your concern.... She has well differentiated keratinizing squamous cell carcinoma.  If her general health is good then treatment of choice is wide excision of carcinoma followed by chemotherapy or radiotherapy if needed. Consult your doctor and take treatment accordingly. Hope I have answered your question, if you have doubt then I will be happy to answer. Thanks for using Chat Doctor. Wish you a very good health.
\\\\
Modified text: I've reviewed your inquiry and understand your concern. It appears she has well-differentiated keratinizing squamous cell carcinoma. If her overall health is good, the preferred treatment is wide excision of the carcinoma, followed by chemotherapy or radiotherapy if necessary. I recommend consulting with your doctor to discuss treatment options and proceed accordingly. If you have any further questions or doubts, feel free to ask. Wishing you good health.
\\\\
Original text: Thank you for using Chat Doctor. I would suggest that you see your doctor. Your baby maybe having bronchiolitis which is a lung infection common to your kids age. It is commonly caused by a virus. Albuterol via nebulization should be utilized in order to alleviate the wheezing and also help with the congestion. A decongestant can also be used for the colds. Also, it would also advise doing a chest X-ray in order to rule out other diseases (ex. pneumonia)sincerely, Mark RosarioGeneral pediatrics/Pediatric Pulmonology
\\\\
Modified text: It sounds like your baby might be experiencing bronchiolitis, a common lung infection among children of their age, typically caused by a virus. To help alleviate the wheezing and congestion, I recommend using Albuterol through nebulization. Additionally, a decongestant can be beneficial for managing cold symptoms. Considering the situation, it would be prudent to consult with your doctor for further evaluation. They may suggest a chest X-ray to rule out other potential conditions, such as pneumonia. Take care.
\\\\
Here's the target text: \texttt{[ORIGINAL RESPONSE]}
\\\\
*Please make sure to thoroughly remove all mentions of ``Chat Doctor'' and person names (e.g., Dear John) from the target text. Also, expressions like ``thank you for your query'' and ``thank you for consulting with us'' are awkward in genuine patient-doctor conversations because these expressions are more appropriate on online platforms; therefore, just remove them or replace them with different expressions that feel more natural and convey empathy. Your response:
\\
\bottomrule
\end{tabular}
\caption{
Example of the input prompt for generating the ChatDoctor-cleaned data.
The ``gpt-3.5-turbo-0613'' checkpoint was used.
}
\label{tab:prompt_chatdoctor_cleaning}
\end{table*}
